Language Fusion for Parameter-Efficient Cross-lingual Transfer

Limited availability of multilingual text corpora for training language models often leads to poor performance on downstream tasks due to undertrained representation spaces for languages other than English. This 'under-representation' has motivated recent cross-lingual transfer methods to leverage the English representation space by e.g. mixing English and 'non-English' tokens at the input level or extending model parameters to accommodate new languages. However, these approaches often come at the cost of increased computational complexity. We propose Fusion forLanguage Representations (FLARE) in adapters, a novel method that enhances representation quality and downstream performance for languages other than English while maintaining parameter efficiency. FLARE integrates source and target language representations within low-rank (LoRA) adapters using lightweight linear transformations, maintaining parameter efficiency while improving transfer performance. A series of experiments across representative cross-lingual natural language understanding tasks, including natural language inference, question-answering and sentiment analysis, demonstrate FLARE's effectiveness. FLARE achieves performance improvements of 4.9% for Llama 3.1 and 2.2% for Gemma~2 compared to standard LoRA fine-tuning on question-answering tasks, as measured by the exact match metric.

==> Tables/results_xquad_detail.tex <==
\begin{table*}
\begin{center}
\scalebox{0.45}{
    % \begin{tabular}{lll>{\columncolor{gray!25}}c*{5}{c}|c}
    \begin{tabular}{ll>{\columncolor{gray!25}}c*{12}{c}|c}
    \hline
    \textbf{Model} &
    \textbf{Fusion Function} &
    \textbf{en} &
    \textbf{ar} &
    \textbf{de} &
    \textbf{el} &
    \textbf{es} &
    \textbf{hi} &
    \textbf{ro} &
    \textbf{ru} &
    \textbf{th} &
    \textbf{tr} &
    \textbf{vi} &
    \textbf{zh} &
    \textbf{Avg.} \\
    \hline

    \hline
    \multicolumn{16}{l}{\textit{Zero-Shot Cross-lingual Transfer}}\\
    \hline
    XLM-R Base & - & 80.73 / 66.78 & 68.31 / 55.97 & 63.80 / 52.02 & 58.36 / 45.80 & 67.01 / 55.38 & 68.66 / 56.55 & 64.25 / 52.27 & 63.62 / 51.85 & 67.21 / 55.38 & 67.30 / 55.21 & 66.45 / 54.71 & 68.44 / 56.55 & - / - \\
    XLM-R Large & - & 85.38 / 72.19 &  70.51 / 59.93 & 70.55 / 61.43 & 69.28 / 60.68 & 79.70 / 71.18 & 74.08 / 63.82 & 74.42 / 67.08 & 69.29 / 58.93 & - / - & 73.75 / 65.42 & 73.03 / 62.67 & 72.16 / 60.00 & & \\
    mT5-XL & - & & & & & & & & & & & & & & \\
    
    \hline
    \multicolumn{16}{l}{\textit{Translate-Test (translate test data to English using NLLB 3.3B)}}\\
    \hline
    
    XLM-R Base & - & - & 67.40 / 57.76 & 68.32 / 58.60 & 65.47 / 56.51 & 76.53 / 66.71 & 72.36 / 62.16  & 70.93 / 63.13 & 67.08 / 56.40 & - / - & 69.55 / 61.18 & 70.32 / 60.76 & 67.41 / 55.40 & \\
    XLM-R Large & - & - & 69.77 / 58.30 & 70.78 / 61.30 & 68.42 / 59.38 & 79.70 / 71.18 & 72.42 / 63.11 & 73.88 / 65.84 & 68.98 / 57.24 & - / - & 72.62 / 63.50 & 73.59 / 63.35 & 70.41 / 57.27 & \\
    mT5-XL & - & - & 68.77 / 59.93 & 69.93 / 61.18 & 67.94 / 60.16 & 78.30 / 69.94 & 73.66 / 64.77 & 74.40 / 66.83 & 70.70 / 59.63 & - / -  & 72.89 / 64.65 & 72.64 / 61.85 & 70.25 / 59.42 & \\
    
    \hline
    \multicolumn{16}{l}{\textit{Translate-Train (models are trained on training data translated to the target language)}}\\
    \hline
    XLM-R Base & - & - & 84.03 / 72.35 & 70.92 / 61.18 & 69.06 / 60.81 & 83.62 / 71.26 & 74.45 / 64.41 & 74.03 / 66.71 & 69.63 / 58.93 & - / - & 73.75 / 65.81 & 73.16 / 63.62 & 71.92 / 59.71 & - \\
    XLM-R Base + Fusion & add relu & - & 82.00 / 70.50 & 81.98 / 70.92 & 82.16 / 71.26 & 81.81 / 70.50 & 81.83 / 70.84 & 81.96 / 70.67 & 82.06 / 70.92 & 81.87 / 70.67 & 82.19 / 71.34 & 81.96 / 70.84 & 82.15 / 71.18 & 82.00 / 70.88 \\
    XLM-R Large & - & - & 84.03 / 72.35 & 83.13 / 71.18 & 69.06 / 60.81 & 83.62 / 71.26 & 74.45 / 64.41 & 74.03 / 66.71 & 69.63 / 58.93 & - / - & 73.75 / 65.81 & 73.16 / 63.62 & 71.92 / 59.71 & \\
    XLM-R Large + Fusion & add relu & -  & 84.42 / 72.52 & 83.71 / 71.76 & 82.34 / 70.67 & 84.71 / 73.19 & 85.22 / 72.86 & 84.26 / 72.35 & 83.54 / 71.60 & 84.55 / 73.19 & 83.88 / 71.60 & 84.35 / 72.18 & 85.42 / 74.03 & - / - \\
    mT5-XL & & & & & & & & & & & & & & & \\
    mT5-XL + Fusion & add relu & - & - / - & 85.76 / 74.71 & & & & & & & & & 87.04 / 76.55  & \\
    
    \hline
    \multicolumn{16}{l}{\textit{Translate-Train (fusion models are trained on training data translated to the target language and evaluated using gold translations in the source language)}}\\
    \hline
    XLM-R Base + Fusion & add relu & - & - / - & - / - & & & & & & & & & & &  \\
    XLM-R Large + Fusion & add relu & & & & & & & & & & & & & & \\
    mT5-XL + Fusion & add relu & & & & & & & & & & & & & & \\
    
    \hline
    \end{tabular}}
    \caption{Average scores per language in XQuAD (F1 / EM). Lora R = 64}
    \label{tab:results_xquad_detail}
\end{center}
\end{table*}
